Distortion results and invariant cantor sets of unimodal maps

A distortion theory is developed for $S-$unimodal maps. It will be used to get some geometric understanding of invariant Cantor sets. In particular attracting Cantor sets turn out to have Lebesgue measure zero. Furthermore the ergodic behavior of $S-$unimodal maps is classified according to a distortion property, called the Markov-property.

==> mark6.tex <==
%auto-ignore
%\magnification=1200
\tolerance=3000

\bigskip
\centerline{\bf 6. The existence of continuous invariant measures}
\bigskip

\flushpar
In this section we will study the existence of absolutely continuous 
invariant measures for $S-$unimodal maps. An initial observation in this 
direction follows from Theorem 5.6: 

\proclaim{Theorem 6.1} If an $S-$unimodal map $f$ has an acim then
$f\in \Cal{I}$. The support of this measure is the topological attractor
which is in this case the orbit of a periodic interval.
\endproclaim

\flushpar
Hence we can restrict ourselves in this section to maps havings the 
Markov-Property. Fix during this section such an $S-$unimodal map $f$. 
Denote its attractor by $A$. 

\bigskip
\flushpar
Using the Markov map we will define a system $(X,F,\hat{\lambda})$ which 
has the unimodal map $f$ as an absolutely continuous factor. This lift will 
always have an acim. The question is whether or not this measure can be 
projected onto an acim for $f$.

\flushpar
Choose $x\in \Cal N$ and consider $M_x:E_x\cap U_x\to U_x$. The collection 
$\Cal{X}$ is formed by subsets of the form $f^i(I)$ where $I$ is a component
of $E_x\cap U_x$ and $0<i\le t_I$. The number $t_I$ is the tranfer time for $I$
to $U_x$. Let $X$ be the set consisting of pairwise disjoint copies of the 
element of $\Cal X$ and let $\pi:X\to [0,1]$ be the corresponding projection 
which is defined by inclusion. In this way every component of $X$ has as 
natural 
measure the Lebesgue measure. The measure $\hat{\lambda}$ on $X$ obtained in 
this way makes $\pi$ absolutely continuous.

\flushpar
The map $f$ can be lifted to a map $F:X\to X$ in a natural way: 
$F|f^i(I)\to f^{i+1}(I)$ for $i<t_I$ is described by the the restriction of $f$
to $f^i(I)$. The defintion of $F$ is extended to every component $I$ of 
$E_x\cap U_x$ such that  $F:I\to f(I)$ equals $f:I\to f(I)$.

\flushpar
Observe that for every $x\in \Cal N$ we defined a new system 
$(X,F,\hat{\lambda})$. Although we supressed in the notation the dependence on
the chosen point in $\Cal N$ the constructed lifts for different points in 
$\Cal N$ will be far from equal.  


\proclaim{Proposition 6.2} The map $F:X\to X$ has the following properties
\parindent=15pt
\item{1)} $\pi \circ F=f \circ \pi$, and the conjugation $\pi$ is absolutely
continuous with respect to $\lambda$ and $\hat{\lambda}$;
\item{2)} $F$ is ergodic and conservative with respect to $\hat{\lambda}$;
\item{3)} $F$ has an acim $\hat{\mu}$ with respect to $\hat{\lambda}$. This 
measure has the additional property that every component of $X$ has finite 
measure;
\item{4)} The measure $\pi_*\hat\mu$ is an absolutely continuous invariant 
measure for
$f$.
\endproclaim
 

\demo{Proof} The map $F$ is constructed in such a way that it projects onto 
$f$. Furthermore the construction made $\pi$ absolutely continous which easily
imply that $\pi_*\hat{\mu}$ is an absolutely continuous invariant measure for
$f$. 

\flushpar
For proving 2) and 3) it is sufficient to remark that the first return map to 
$U_x\subset X$ corresponding to $F:X\to X$  is described by the Markov map 
$M_x:U_x\cap E_x\to U_x$.

\flushpar
The ergodicity and conservativity follows directly by using the uniform bounded
distortion property of the branches of the iterates of $M_x$. 

\flushpar
We obtain an acim for $F$, having the additional property, by applying results 
from [M2]. An other way for obtaining an acim for $F$ is using the well know 
existence of an acip for $M_x:E_x\cap U_x\to U_x$, the return map to 
$U_x\cap X$. 
\qed
\enddemo


\flushpar
The main question left over is whether the absolutely continuous invariant 
measure $\pi_*\hat{\mu}$ for $f$ is  relevant; finite or $\sigma-$finite.
A related question is whether every acim for $f$ is of the 
form $\pi_*\hat{\mu}$. The remaider of this section will be devoted to the 
question whether or not the measure $\hat{\mu}$ can be projected to acim 
for $f$ . 

\flushpar
Denote the return map to a set 
$D\subset X$ with $\hat{\lambda}(D)>0$ by $F_D:D \to D$. The conservativity of 
$F$ assures that this return map is almost everywhere defined. Furthermore let 
the function $s:X\to\bold{R}$ be given by 
$$
s(x)=|I|,
$$
where $I\subset X$ is the component of $X$ containing $x$. Observe that this 
function is bounded and everywhere positive. The mean value along
orbits will give us information about the measure $\hat{\mu}$. Consider for 
every set $D\subset X$ with positive measure the function 
$\overline{s}_D:X\to \bold{R}$ defined by 
$$
\overline{s}_D(x)=
\limsup_{n\to \infty}
\frac1n \sum_{j=0}^{n-1} s(F^j_D(x)).
$$
The ergodicity of $F$ implies that the function $\overline{s}_D$ are in fact 
almost everywhere equal to a constant $\overline{s}_D\ge 0$. 

\proclaim{Lemma 6.3} For every $D\subset X$ with positive measure we have
$$
\overline{s}_D>0  \text{ if and only if } \hat{\mu}(D)<\infty.
$$
\endproclaim

\demo{Proof} If $\hat{\mu}(D)<\infty$ then the return map $F_D$ has an acip:
$\frac{\hat{\mu}|D}{\hat{\mu}(D)}$. The return map $F_D$ is ergodic. Hence by
using the Egodic Theorem we get
$$
\overline{s}_D=\frac{\int_D s d\hat{\mu}}{\hat{\mu}(D)}>0.
$$ 
Suppose on the otherhand that $\overline{s}_D>0$. Now let 
$G=s^{-1}((\frac12 \overline{s}_D,\infty))$: $G$ consists of the components $I$
of $X$ with $|I|>\frac12 \overline{s}_D$. The contraction principle implies 
that $G$ consists of finitely many such components. Hence,using 
Lemma 6.2(3),
$$
\hat{\mu}(G)<\infty.
$$
Take $x\in D$ with $\overline{s}_D=\overline{s}_D(x)$ and consider
$$
\aligned
\overline{s}_D&=\overline{s}_D(x)=
                \limsup_{n\to \infty}
                \frac1n \sum_{j=0}^{n-1} s(F^j_D(x))\\
              &=\limsup_{N\to\infty}
                \frac{\sum_{j=0}^N s(F^j(x)\bold{1}_D(F^j(x))}
                     {\sum_{j=0}^N \bold{1}_D(F^j(x))}\\
              &=\limsup_{N\to\infty}
                \frac{\sum_{j=0}^N s(F^j(x))\{\bold{1}_{D\cap G}(F^j(x))+
                                             \bold{1}_{D\cap (X-G)}(F^j(x))\}}
                     {\sum_{j=0}^N \bold{1}_D(F^j(x))}\\
              &\le \limsup_{N\to\infty}
                   \frac{\sum_{j=0}^N \bold{1}_{D\cap G}(F^j(x))}
                        {\sum_{j=0}^N \bold{1}_D(F^j(x))}+
                   \frac12\overline{s}_D 
                   \limsup_{N\to\infty}
                   \frac{\sum_{j=0}^N \bold{1}_{D\cap (X-G)}(F^j(x))}
                        {\sum_{j=0}^N \bold{1}_D(F^j(x))}\\
              &\le \frac{\hat{\mu}(D\cap G)}{\hat{\mu}(D)}+
                   \frac12 \overline{s}_D. 
\endaligned
$$ 
The last inequality is obtained by using the Chacon-Ornstein theorem which is
possible because $\hat{\mu}(D\cap G)<\infty$. Hence
$$
\hat{\mu}(D)\le \frac{2\hat{\mu}(D\cap G)}{\overline{s}_D}<\infty.
$$
\qed 
\enddemo

\flushpar
The next step is to relate the numbers $\overline{s}_D$ to observable 
quantities of the system $f$. For this we go back to the functions $r_n$ 
defined in section 5.
Let $D$ be a subset of the topological attractor of $f$ with positive Lebesgue 
measure. And let $f_D:D\to D$ be the corresponding retrurn map 
which is almost everywhere defined, $f$ is conservative on its attractor.

\flushpar
Define the function $r_{D,n}:D\to \bold{R}$ by
$$
r_{D,n}(x)=r_{t_n}(x)
$$
where $t_n$ is defined by $f_D^n(x)=f^{t_n}(x)$. To describe the limit
behaviour of these function we introduce $\overline{r}_D:D\to \bold{R}$ where
$$
\overline{r}_D(x)=\limsup_{n\to \infty}\frac1n \sum_{j=0}^{n-1} r_{D,j}(x).
$$
Again, by the ergodicity of $f$, these function are almost everywhere equal
to a constant, say $\overline{r}_D\ge 0$. 

\proclaim{Theorem 6.4} Let $f\in \Cal I$ with attractor $A$.
\parindent=15pt
\item{1)} $\overline{r}_A>0$ if and only if $\pi_*\hat\mu$ is an acip for $f$;
\item{2)} $\overline{r}_A=0$ and $\overline{r}_D>0$ for some $D\subset A$
with positive Lebesgue measure if and inly if $\pi_*\hat\mu$ is an infinite 
acim for $f$.
\endproclaim

\flushpar






\flushpar
In a forthcoming paper we will show that every $\sigma-$finite (or finite) 
absolutely continuous invariant 
measure for $f$ is the projection of the absolutely continuous invariant measure
on $\hat{X}$. This implies that the above stated sufficient conditions for the 
existence of absolutely continuous invariant measures are in fact also 
nescessary.

\flushpar
All the results are stated for $S-$unimodal maps. In fact it can be shown that 
the orbits of the intervals considered in the proofs of section 3
satisfy the neccesary disjointness conditions needed for applying the 
$C^2-$Koebe-Lemma. Hence the results in this section also hold for 
$C^2-$unimodal maps. The difficulties for proving the $C^2$ versions of the 
Theorems in this 
paper occur when dealing with the orbits of TI-pairs. These orbits do not 
satisfy some disjointness conditions needed for applying the $C^2-$Koebe-Lemma. 
However the intervals in these orbits are nested, as described by Lemma 2.7.
This property makes it possible to make the nessasary estimates for 
applying the $C^2$-Koebe-Lemma. All results stated in this paper will turn out
to be true for $C^2$-unimodal maps.

